Switching Controller Synthesis for Delay Hybrid Systems under Perturbations

Delays are ubiquitous in modern hybrid systems, which exhibit both continuous and discrete dynamical behaviors. Induced by signal transmission, conversion, the nature of plants, and so on, delays may appear either in the continuous evolution of a hybrid system such that the evolution depends not only on the present state but also on its execution history, or in the discrete switching between its different control modes. In this paper we come up with a new model of hybrid systems, called \emph{delay hybrid automata}, to capture the dynamics of systems with the aforementioned two kinds of delays. Furthermore, based upon this model we study the robust switching controller synthesis problem such that the controlled delay system is able to satisfy the specified safety properties regardless of perturbations. To the end, a novel method is proposed to synthesize switching controllers based on the computation of differential invariants for continuous evolution and backward reachable sets of discrete jumps with delays. Finally, we implement a prototypical tool of our approach and demonstrate it on some case studies.

==> linear.tex <==
\section{The Synthesis Algorithm for Linear Systems}\label{sec:linear}

\YB{ Another a version in different structure, 
please see https://www.overleaf.com/5499635344vmfvqwtjfzzp.
Which structure is better? If that, I will modify this repo.}


In this section, 
we consider the linear sub-class of systems given in DDE \eqref{dde:DDE}:
\begin{equation}\label{dde:linearDDE} 
    \left\{  
                 \begin{array}{lr}  
                 \dot{\bm{x}}(t)= A\bm{x}(t) + B \bm{x}(t-r) + C \bm{w}(t), & t\in [0,\infty) \\  
                 \bm{x}(t)= \bm{\phi}(t) , & t\in [-r,0]
                 \end{array}  
    \right.  
\end{equation}
 where $A, B\in \mathbb{R}^{n\times n}$, $C \in \mathbb{R}^{n\times m}$ are real matrices of appropriate dimensions.
We  present our high-level synthesis algorithm and the subroutines that are used herein for solving switching
controller synthesis problem. 
\emph{Differential invariant} generation and backward reachable set computation are the key methods, which are introduced in details then.

\begin{definition}[Global Ball-convergence]\label{def:ball_convergence}
    Given system \eqref{dde:linearDDE}, assume that $\bm{x}_e$ is an equilibrium, i.e. $\bm{f}(\bm{x}_e, \bm{x}_e) =\bm{0}$.
    For a given $\mathfrak{r} >0$, system \eqref{dde:linearDDE} is called to be globally exponentially convergent within the ball
    $\mathfrak{B}(\bm{x}_e, \mathfrak{r})$ if there exists a constant $\alpha > 0$ and non-decreasing function$\beta(.)$
    such that the following condition holds:
    \begin{equation*}
        \| \bm{\xi}_{\bm{\phi}}(t) - \bm{x_e} \| \leq \mathfrak{r} + \beta(\| \bm{\phi}\|)\mathrm{e}^{-\alpha t}, t\geq 0,
    \end{equation*}
    for all $\bm{\phi}\in \mathcal{C}\{ [t_1, t_2], \mathbb{R}^n\}$ and $\| \bm{w}(t) \| \leq w_{max}$.
\end{definition}
In Definition \ref{def:ball_convergence}, $\alpha$ represents rate of decay, i.e. an estimate of how 
quickly the solution of system \eqref{dde:linearDDE} converges to the ball $\mathfrak{B}(\bm{x}_e, \mathfrak{r})$.
Especially, when the radius of the ball $\mathfrak{r}=\bm{0}$, the definition of ball convergence is consistent with 
Lyapunov exponential stability \cite{Lyapunov_stability}. 

\subsection{Differential Invariant Generation}\label{subsec:boundTsec}

\begin{definition}[Differential invariant]\label{def:diff_invariant}
Given a mode $q\in Q$ of a delay hybrid automaton $\mathcal{H}$: $(\Xi(q), \bm{f}_q, I(q))$ and time $T$, a set $I^*$ is called a $T$- invariant,
if for any trajectories starting from a given initial function $\bm{\phi}_q \in \Xi(q)$, the following
condition holds:
\begin{equation}
    \forall t\in [-r_q, T], \  \bm{\xi}_{\bm{\phi}_q}(t) \in I(q) \rightarrow \bm{\xi}_{\bm{\phi}}(t)\in I^*(q). 
\end{equation}
\end{definition}

$T$- invariant $I^*(q)$ requires that every trajectory starting from initial states 
in time $T$ remains  inside the differential invariant $I^*(q)$ if it remains inside the domain $I(q)$. 
If $T=\infty$, then $I^*(q)$ is a differential invariant of mode $q$.
Moreover, a  differential invariant $I^*(q)$ is \emph{safe} iff $I^*(q) \subseteq \mathcal{S}_q$.

One of our main contributions is a two-steps procedure to  generate the differential invariant for each mode $q$ of the delayed hybrid 
system $\mathcal{H}$. The first step is to calculate a bounded horizon $T$ using ball convergence analysis, which reduces the differential invariant problem into the $T$-differential invariant problem.
After attaining a bounded time $T$, the task of the second step is to compute a reachable set in time $T$. 
Let us take a look at the first step of the differential invariant generation.

In \cite{trinh2014new}, a class of linear DDE systems has been studied that 
under perturbation, there exists a ball to bound all state trajectories from some region of initial conditions,
and for the other part of initial conditions, all state trajectories from it converge 
exponentially within the ball. First,  we recall the theorem in the following:
\begin{theorem}[\cite{trinh2014new}]
\label{thm:expenential}
Let $M=A+B$ be a Metzler matrix, then there exist positive constants 
$\beta$, $\gamma$, $\delta$, $\eta$ such that for all initial functions $\bm{\phi}$, the following condition holds:
\begin{equation}
    \| \bm{\xi}_{\bm{\phi}} \|_{\infty} \leq \frac{C_{max} w_{max}}{\eta} + \beta ( \|\bm{\phi} \|_{\infty} -\frac{C_{max} w_{max}}{\delta})^+ \mathrm{e}^{-\gamma t}
\end{equation}
where $C_{max} = \max_{i\in n} \sum_{j}^{m} C_{ij} $.
\end{theorem}

In Theorem \ref{thm:expenential}, with the term of the Metzler matrix, the system \ref{dde:linearDDE}
is globally exponentially convergent to the ball $\mathfrak{B}(\bm{0}, \frac{C_{max} w_{max}}{\eta})$
for all perturbation $\| w\|_{\infty} \leq w_{max}$. Moreover, the size of the ball  increases as the perturbation bound
increases. 
Particularly, without perturbation by letting $w(t) =0$ for all $t\in [-r_k, \infty)$, the system 
is globally exponential stable to the equilibrium $\bm{0}$. The construction of the positive constants can be done 
in the following way: define a $\zeta \geq \bm{0}$ such that $\| \zeta \|_{\infty}=1$ and $\zeta M \leq \bm{0}$,
then 
	 $\beta=(\zeta)^{-1}_{min}$,
	 $\eta=(-M\zeta)_{min}$, 
	 $\delta=\eta (\zeta)^{-1}_{min}$,
	 $\gamma=\min_{i} \gamma_i$ such that $\gamma_i$ is the solution of the equation
	 \begin{equation*}
		 H_i(\gamma) = \gamma \zeta_i +\sum_{j=1}^n \zeta_j b_{ij}(e^{\gamma r_k - 1}) - \eta = 0  .
	 \end{equation*}
Utilizing the character of globally exponential converging to a ball, a finite bound $T\in \mathbb{R}^+$ can be calculated
by the following theorem:
\begin{theorem}
\label{thm:reduceT}
Given an initial function $\bm{\phi}$ and the equilibrium $\bm{x_e}=\bm{0}$,
if we know $\beta$, $\gamma$, $\delta$ and $\eta$, let $\mathfrak{r}_1=\frac{C_{max} w_{max}}{\eta} $ and $\mathfrak{r}_2 = \beta ( \|\bm{\phi} \|_{\infty} -\frac{C_{max} w_{max}}{\delta})$, then for any given $\epsilon >0$,
there exists a time bound $T^*$ defined by 
\begin{equation}
    T^* = \max\{ 0, \inf \{ T \mid \forall t\geq T : \mathfrak{r}_2^+ \mathrm{e}^{-\gamma t}<\epsilon \}\}
\end{equation}
the solution of systems \ref{dde:linearDDE} satisfies: for any $T \geq T^*$, 
$\|\bm{\xi}_{\bm{\phi}}(T)-\bm{x_e}\|_{\infty}- \mathfrak{r}_1 < \epsilon$,
then the differential invariant of the system \ref{dde:linearDDE} is equivalent to 
$T$-differential invariant. 
\end{theorem}
\begin{proof}
	For the \emph{necessity} part, because the differential invariant implys $T$-differential invariant by Definition \ref{def:diff_invariant}, the proof is for free.
	For the \emph{sufficiency} part, by Theorem \ref{thm:expenential}, $\| \bm{\xi}_{\bm{\phi}} \|_{\infty} \leq \mathfrak{r}_1 + \mathfrak{r}_2^+ \mathrm{e}^{-\gamma t} $
	for any $t\geq 0$ and $\bm{\phi}$. Moreover, $\mathfrak{r}_2^+ \mathrm{e}^{-\gamma t}$  is strictly monotonically decreasing w.r.t $t$,
	hence there exists a upper bound $T^*$ such that for any $t\geq T^*$, $\mathfrak{r}_2^+ \mathrm{e}^{-\gamma t}$ is exponentially close to equilibrium $\bm{x}_e$ within 
	a accuracy $\epsilon$. Therefore given a accuracy $\epsilon$, for any $t\geq T^*$, all trajectories starting from $\bm{\phi}$ are exponentially converging to the ball $\mathfrak{B}( \bm{x_e}, \mathfrak{r}_1 )$.

\end{proof}


%\subsection{Safe reachable set computation in T}\label{reachsec}
Theorem \ref{thm:reduceT} sets up a sound guarantee that a differential invariant problem can be reduced to a $T$-differential invariant problem.
Now it is ready to introduce the second step of the differential invariant generation.
In order to solve $T$-invariant generation problem of DDEs, we adapt the  method \cite{Reissig2016} for ODEs to compute a safe over-approximation reachable set of the system \eqref{dde:linearDDE} from the initial set. 
The over-approximation of the reachable set is formalized by a \emph{growth bound}.

\begin{definition}[Growth bound]
	Given a time $t$ and a set $K \subset I(q)$, a growth bound is a map 
	$\Lambda_t: \mathbb{R}^n_{+} \rightarrow \mathbb{R}^n_{+}$ 
	satisfying the following conditions:
	\begin{itemize}
		\item $\Lambda_t(\rho) \geq \Lambda_t(\rho')$ whenever $\rho \geq \rho'$,
		\item $\xi$ is a trajectory of system \eqref{dde:linearDDE}  
		 on $[-r,t]$ with $y,x \in K$, then 
		 \begin{equation*}
			|\xi_y(t) - \xi_x(t) | \leq \Lambda_t(|y -x |)
		 \end{equation*}
		where $\xi_x(t)$ denotes the trajectory starting from $x$ with respect to the system \eqref{dde:linearDDE}.
	\end{itemize}
\end{definition}

We now present a specific way to compute the growth bound $\Lambda_t(\cdot)$:

\begin{theorem} %computation of growth
 \label{thm:computeGrowth}
	Given a system \eqref{dde:linearDDE},  let $t>0$, $\mathfrak{r} \in \mathbb{R}^n_+$, the map $\Lambda_t$ is given by:
	\begin{equation}
		\Lambda_t (\mathfrak{r}) =   \mathrm{e}^{L t} \mathfrak{r} + \int_{0}^{t} \mathrm{e}^{Ls} |B|\mathfrak{r}(s-r)  \mathrm{d}s
	\end{equation}
	where the matrix $L$ satisfies 
	\begin{equation*}
		L_{ij} \geq 
		\left\{
             \begin{array}{lr}
             A_{ij}, &  i=j  \\
             |A_{ij}|, & \text{otherwise} 
             \end{array}
\right.
	\end{equation*}
\end{theorem}
\begin{proof}
Given any states $x(t),y(t) \in I(q)$, 
let $z(t) = y(t)-x(t) $.
From the system \eqref{dde:linearDDE}, we have
\begin{equation*}
     \dot{z}(t) = \dot{y}(t) - \dot{x}(t)
             =  A z(t) + B z(t-r).
\end{equation*}
Hence, by Lemma 6 in \cite{Reissig2016}, we have
\[ |z(t)| \leq  \mathrm{e}^{L t} \mathfrak{r} + \int_{0}^{t} \mathrm{e}^{Ls} |B|\mathfrak{r}(s-r)  \mathrm{d}s. \]

\end{proof}

We consider the discretization of the initial states set defined by hyper-rectangle covers.
A \emph{hyper-rectangle} $[\![a,b]\!]$ with $a,b\in (\mathbb{R}\cup\{\pm\infty\})^n$ 
defines the set $\{x \in\mathbb{R}^n\mid a_i \leq x_i\leq b_i  \text{for} i\in\{1,\ldots,n\}\}$;
it is non-empty if $a < b$ (element-wise).
For $\rho \in \mathbb{R}^n_{+}$, we say that a hyper-rectangle $[\![ a,b]\!]$
has diameter $\rho$ if $| b - a| = \rho$, where $|\cdot |$ represents the element-wise absolute value.
The \emph{center} of a non-empty hyper-rectangle $[\![ a, b]\!]$, written $ctr( [\![ a,b]\!])$, 
is the point $(\frac{1}{2}(b_1-a_1), \frac{1}{2}(b_2 - a_2), \ldots, \frac{1}{2}(b_n - a_n))$.
% A set $C$ of hyper-rectangles is called a \emph{cover} of the state space $X$ if
% every $x\in X$ belongs to some hyper-rectangle in $C$.
For each hyper-rectangle of the initial set, a over-approximate reachable set is obtained by growth bound in Theroem \ref{thm:computeGrowth}. 


\subsection{Backward Reachable Set Calculation}\label{subsec:backsec}
For each mode $q$ of the delay hybrid automaton $\mathcal{H}$. a differential invariant $I^*(q)$ can be computed by employing the techniques in Section \ref{subsec:boundTsec}.
Then, for each edge $e=(q, q')\in E$, 
a \emph{fake} switching controller can be calculated as $\widetilde{G}(e) = I^*(q) \cap G(e)$, where a \emph{fake} switching controller 
refers to the one without considering the delay $D(e)$ at $e$ edge.
To address a \emph{real} switching controller $G^*(e)$ with regard to the delay $D(e)$, 
we treat the \emph{fake} controller $\widetilde{G}(e)$ as the target set, and search for a set $G^*(e)$ such that all trajectories  starting from the set $G^*(e)$ will reach into $\widetilde{G}(e)$  after the duration time $D(e)$. 
Our another contribution is to formalize this notion as the following definition and introduce a method to calculate the set $G^*(e)$. 

\begin{definition}[Backward reachable set]
	\label{def:backreachset}
	For a mode $q$ of the delay hybrid automaton $\mathcal{H}$ : $(\Xi(q), \bm{f}_q, I^*(q))$, 
	given a target region $\widetilde{G}(e)$ and a finite time $t=D(e)$, a backward reachable set 
	$G^*(e)$ of the target region $\widetilde{G}(e)$ at time $t=0$ is defined as follows:
	\begin{equation*}
	    	G^*(e) = 
	    	\left\{ \bm{x} \in \mathbb{R}^n \,\middle|\,
	    	\begin{array}{cc}
	    	    &\forall t\in [0,D(e)] , \forall \bm{w}:\\
	    	    &\xi_{\bm{x}} (D(e)) \in \widetilde{G}(e) \wedge 
	    	    \xi_{\bm{x}}(t) \in I^*(q)  
	    	\end{array}
	    	\right\}.
	\end{equation*} 
\end{definition}

Definition \ref{def:backreachset} describes
a set that all trajectories  starting from  at time $t=0$ will reach the given target
set after a given time $t=D(e)$, while all possible trajectories stay in the domain during the 
time interval $[0,D(e)]$, despite the uncertain actions of perturbation.
And the set $G^*(e)$ in Definition \ref{def:backreachset} is a \emph{real} switching controller.
As the best of our knowledge, few approaches have been developed to calculate the backward reachable set for DDEs. One option is to seek for all states in the invariant 
but this may be wasteful if, e.g., only a small part of state space is able to reach the target region.
We come up with a local algorithm to search for the backward 
reachable set locally instead of a global search.

\begin{remark}
explain why the initial state here is a state not a function.
\end{remark}

%discretization
Given a discretization parameter $\rho \in \mathbb{R}^n_{+}$, we donate $\widehat{I}^*(q)$ as the discretization of  $I^*(q)$ that is the cover of it with rectangles
of diameter $\rho$.
%maximal boundary
For parameters $\rho$ and $t=D(e)$, define a set $\widehat{S} = [\![-s,s]\!]$,  where 
$s$ is a $n$-dimensional vector defined by $s=\lceil \sup_{\bm{x},\bm{w}} \bm{f} \rceil \cdot D(e)/ \rho$.
In time $D(e)$, whether a trajectory from a state can reach into $\widetilde{G}$ depends on the speed of underlying system dynamics. We inflates the boundary of $\widetilde{G}$ with an extend of 
$\widehat{S}$ by an operator $\uplus$ : 
\begin{equation*}
    \widetilde{G}(e) \uplus \widehat{S} = 
    \left\{ \widehat{\bm{x}} \in \widehat{I}^*(q) \,\middle |\,
    \begin{array}{cc}
        \exists \widehat{\bm{x}}'\in \widetilde{G}(e), 
	    \exists  \widehat{\bm{y}}\in \widehat{S}: \\
	    ctr(\widehat{\bm{x}}) = ctr(\widehat{\bm{x}}') + \widehat{\bm{y}}\cdot D(e) 
    \end{array}
	\right\}.
\end{equation*}
Then all trajectories starting from  the set $\widehat{I}^*(q) \setminus (\widetilde{G}(e) \uplus \widehat{S})$ are not possible to reach into $\widetilde{G}(e)$ in time $D(e)$.
Therefore, we only need to consider the set $\widetilde{G}(e) \uplus \widehat{S}$.
For each abstract state $\widehat{x} \in \widetilde{G}(e) \uplus \widehat{S}$, its over-approximate reachable set is calculated and checked whether it stays in $I^*(q)$ and all reachable states $\bm{x}(D(e))$ reach into $\widetilde{G}(e)$. If the answer is \emph{yes}, then retain it. 
Otherwise, if only some of reachable states $\bm{x}(D(e))$ reach into $\widetilde{G}(e)$, then refine the abstract state $\widehat{\bm{x}}$ using a smaller discretization parameter $\rho'$, e.g. $\rho'=\rho/2$. 
Continue this process until  all abstract states  are done in the set $\widetilde{G}(e) \uplus \widehat{S}$.
Algorithm \ref{alg:backreachset}  summarizes this approach.


\begin{algorithm}
	\caption{BackwardReach}
\begin{algorithmic}[1]
\REQUIRE~~
	 $\widetilde{G}(e)$,   $D(e)$,   $I^*(q)$, $\rho$ \\
\ENSURE~~
	$G^*(e)$.
  \STATE $G^*(e) = \emptyset$;
  \STATE $\widehat{I}^*(q) \leftarrow$ a cover of $I^*(q)$ with parameter $\rho$;
  \FOR {each $\widehat{\bm{x}} \in \widetilde{G}(e) \uplus \widehat{S}$}
	 \STATE compute $\bm{x}(t) $ for $t\in [0, D(e)]$
	 \IF{$\bm{x}(D(e))  \subseteq \widetilde{G}(e) \wedge \bm{x}(t)\in I^*(q), \forall t\in [0, D(e)]$ }
		\STATE $G^*(e) \leftarrow G^*(e) \cup \widehat{\bm{x}} $
	 \ELSE \IF{$\bm{x}(D(e))  \cap \widetilde{G}(e) \neq \emptyset$}
		 \STATE refine $\widehat{\bm{x}}$ with $\rho = \rho/2$
	  \ENDIF
	 \ENDIF
  \ENDFOR
  \RETURN $G^*(e)$;
\end{algorithmic}
\label{alg:backreachset}
\end{algorithm}



\subsection{Main Synthesis Framework}

Our main synthesis framework (Algorithm \ref{alg:switch_controller}) is based on the \emph{inductive invariant} on each mode $q$, to obtain a non-trivial switching controller if it exists. The definition of the inductive invariant is as follows:
\begin{definition}[Inductive invariant]
    Given a delay hybrid automaton $\mathcal{H}$, $I^* = \cup_{q\in Q} I^*(q)$ is inductive invariant of $\mathcal{H}$,
    if $I^*$ satisfies the following two conditions:
    \begin{itemize}
        \item[(c1)] for each $q\in Q$, the set $I^*(q)$ is a differential invariant of $(\Xi(q), \bm{f}_q, I(q))$,
        \item[(c2)] for each $e=(q, q')\in E$, if $\bm{\xi}_{\bm{\phi}_q} (t) \in I^*_q \cap G(e)$,
         then for all $\tau\in [t'-r_{q'}, t']$, 
         \begin{equation*}
              \bm{\phi}_{q'}(\tau) \in I(q') \rightarrow \bm{\phi}_{q'}(\tau)\in I^*(q') ,
         \end{equation*}
         where $\bm{\phi}_{q'}(\cdot) = R(e, \bm{\xi}_{\bm{\phi}_q}(t+D(e)))$ and $t'=t+D(e)$.
    \end{itemize}
    \label{def:inductive_invariant}
\end{definition}




Algorithm \ref{alg:switch_controller} presents the synthesis framework for solving the switching controller problem of delayed hybrid systems.
First, for each mode $q\in Q$, we generate its safe differential invariant by the methods introduced in subsection \ref{subsec:boundTsec} (line 2). 
Based on the safe differential invariant, we refine the initial state set $\Xi$, continuous functions set $U$ by intersecting with invariant and safe requirement (lines 3- 5). 
By Definition \ref{def:inductive_invariant}, we extract the reset functions $R^*$ from the original reset functions $R$ (line 11), and collect the states of being reset in $R^*$ as 
\emph{fake} guard conditions (line 12). 
This \emph{fake} guard conditions are the ones without considering any delays in discrete transitions.
Furthermore, in order to deal with the delays in discrete transitions,
new guard conditions are calculated by the backward reachable set search with respect to  the fake guard conditions (line 13).

\begin{algorithm}
\caption{SynthesisFramework}
 \begin{algorithmic}[1]
 \REQUIRE ~~ 
 $\mathcal{H}=(Q, X, U, I, \Xi , F , E, D, G, R )$, $\mathcal{S}$;
 \ENSURE~~
 $\mathcal{H^*}$;
	\FOR{$q\in Q$}
		\STATE \text{compute the invariant} $I^*(q)$; \COMMENT{\textcolor{blue}{subsection} \ref{subsec:boundTsec}}
	    \STATE $\Xi^*(q) \leftarrow \Xi(q) \cap \mathcal{S}_q$;
	    \STATE $I^*(q)\leftarrow I^*(q)\cap I(q) \cap \mathcal{S}_q $;
	    \STATE $U^*_q \leftarrow \{\bm{\phi}\in U \mid \bm{\phi}\in I^*(q) \}$;
	\ENDFOR
	\STATE $\Xi^* \leftarrow \{ (q,\Xi^*(q)) \mid q\in Q\}$;
	\STATE $I^* \leftarrow \{(q,I^*(q))\mid q\in Q\}$;
	\STATE $U^* \leftarrow \{(q, U^*_q)\mid q\in Q\}$;
	\FOR{$e=(q,q')\in E$}
	    \STATE $R^*(e,\cdot) \leftarrow \{ \bm{\phi}_{q'}(\cdot)\in R(e, \cdot) \mid  \bm{\phi}_{q'}(\tau) \in I(q') \rightarrow \bm{\phi}_{q'}(\tau)\in I^*(q') \text{for any}\tau\in [-r_{q'},0]\}$;
	    \STATE $\widetilde{G}(e) \leftarrow \{\bm{x}\in G(e) \cap I^*(q) \mid \bm{\phi}_{q'}(\cdot)= R^*(e,\bm{x}) \}$;
		\STATE \text{compute} $G^*(e)$ \text{backward reachable set search from}  $\widetilde{G}(e)$; \COMMENT{\textcolor{blue}{subsection} \ref{subsec:backsec}}
	\ENDFOR 
	\STATE $G^* \leftarrow \{(e,G^*(e)) \mid e\in E \}$;
	\STATE $R^* \leftarrow \{R^*(e,\cdot) \mid e\in E\}$;
	
	\IF {$\forall e\in E, G^*(e) \neq \emptyset$ }
	    \RETURN $\mathcal{H^*}\leftarrow (Q, X, U^*, I^*, \Xi^* , F , E,D, G^*, R^* )$
	\ENDIF
 \end{algorithmic}
\label{alg:switch_controller}
\end{algorithm}

\begin{example}
We continue to consider the heating system in the motivating example and try to solve it by the approach introduced above. 
Let $K_1=0.25$, $K_2=0.15$ and $h=8$ for delay hybrid automaton of the heating system in Example \ref{exm:heating_automaton}. For mode $q_1$, $M=-0.1$ is trivially a Metzlar matrix. 
Applying the theorem \ref{thm:reduceT}, we have $T^*_{q_1} = 60.587$s. And we obtain its over-approxiamte reachable set in $T^*_{q_1}$ as its differential invariant $I^*(q_1) = \{x \mid 50 \leq x\leq 80\}$, demonstrated in Fig \ref{fig:heatingreach1}. 
The same procedure goes to mode $q_2$, we have $T^*_{q_2}= 60.043$s, and its over-approximate reachable set displayed in Fig \ref{fig:heatingreach2}. The differential invariant is $I^*(q_2) = \{x \mid 50 \leq x\leq 80\}$. 
The switching controllers on $e_1$ and $e_2$ are easily computed as $G^*(e_1) = G^*(e_2)=\{x \mid 50 \leq x\leq 80\}$. Furthermore, Fig \ref{fig:heating_trajectory} depicts several trajectories of the heating system under the safe switching controllers.

\end{example}

\begin{figure}[ht]
    \centering
    \subfigure[]{
        \label{fig:heatingreach1}
    \includegraphics[width=4.3cm, height=3.8cm]{figures/heating.eps}
    }
    \hspace{-7mm}
    \subfigure[]{
        \label{fig:heatingreach2}
    \includegraphics[width=4.3cm,height=3.8cm]{figures/heating2.eps}
    }
    \caption{Over-approximate reachable sets for two modes of the heating system.}  
 \end{figure}
 
 \begin{figure}[ht]
     \centering
     \includegraphics[width=5cm]{figures/trajectory.pdf}
      \captionsetup{justification=centering}
     \caption{The trajectories under the safe \\switching controller for the heating system}
     \label{fig:heating_trajectory}
 \end{figure}

==> nonlinear.tex <==
\section{Synthesis for Nonlinear Systems}\label{sec:nonlinear}
In this section, we generalize the Algorithm \ref{alg:switch_controller} for  nonlinear systems, by means of linearization techniques and dynamics estimation. 
We introduce a new theory in the first step of the differential invariant generation for nonlinear systems, other procedures in  Algorithm \ref{alg:switch_controller} are also applicable to nonlinear systems.
Therefore, in the following, we emphasize how to reduce $\infty$-invariant generation problem to $T$-invariant generation problem for a nonlinear system. 

%linearization
Define 
\begin{equation*}
    A= \left.\frac{\partial \bm{f}}{\partial \bm{x}(t)}\right|_{(\bm{0},\bm{0})} \text{and} \
    B = \left.\frac{\partial \bm{f}}{\partial \bm{x}(t-r)} \right|_{(\bm{0},\bm{0})}
\end{equation*}
to be the Jacobian matrices of $\bm{f}(\bm{x}(t), \bm{x}(t-r))$ with respect to $\bm{x}(t)$ and $\bm{x}(t-r)$, evaluated at the equilibrium $(\bm{0},\bm{0})$.
We get the linearized form of DDE \eqref{dde:DDE} with one single delay term (for the sake of cleaner presentation):
\begin{equation}
\label{dde:linearization_higher}
 \left\{  
                 \begin{array}{lr}  
                 \begin{aligned}
                      \dot{\bm{x}}(t)= A\bm{x}(t) + B \bm{x}(t-r) + C \bm{w}(t) \\
                      + \bm{g}(\bm{x}(t),\bm{x}(t-r)),  
                 \end{aligned}
                 & t\in [0,\infty) \\ 
                 \bm{x}(t)= \bm{\phi}(t) , & t\in [-r,0],
                 \end{array}  
    \right.
\end{equation}
where $\bm{g}$ is the higher-order term, and it will be very closed to zero for $\bm{x}$ sufficiently close to the equilibrium. 
By dropping the higher-order term in DDE \eqref{dde:linearization_higher}, we can obtain the approximation of DDE \eqref{dde:DDE}, which is exactly the same linear system specified in DDE \eqref{dde:linearDDE}.

%local exponential ball convergence (theorem and proof)
\begin{definition}[Local Ball-convergence]
 Given system \eqref{dde:DDE}, assume that $\bm{x}_e$ is a equilibrium, i.e. $\bm{f}(\bm{x}_e, \bm{x}_e) =\bm{0}$.
    For a given $\mathfrak{r} >0$, system \eqref{dde:DDE} is called to be locally exponentially convergent within the ball
    $\mathfrak{B}(\bm{x}_e, \mathfrak{r})$, if there exist a constant $\alpha > 0$ and non-decreasing function$\beta(.)$
    such that for all  $\| \bm{w}(t) \| \leq w_{max}$, the following condition holds:
    \begin{equation*}
       \| \bm{\phi}(t) - \bm{x_e} \|\leq \iota \implies \| \bm{\xi}_{\bm{\phi}}(t) - \bm{x_e} \| \leq \mathfrak{r} + \beta(\| \bm{\phi}\|)\mathrm{e}^{-\alpha t}, t\geq 0.
    \end{equation*}
\end{definition}


\begin{theorem}
\label{thm:expenential_nonlinear}
Let $M=A+B$ is a Metzler matrix, then there exist positive constants 
$\beta$, $\gamma$, $\delta$ and $\eta$ such that for all initial functions $\bm{\phi}$, the following condition holds:
\begin{multline}
          \| \bm{\phi}(t) - \bm{x_e} \|\leq \iota \implies \\
      \| \bm{\xi}_{\bm{\phi}} \|_{\infty} \leq \frac{\mathcal{G}}{\eta} + 
      \beta ( \|\bm{\phi} \|_{\infty} -\frac{\mathcal{G}}{\delta})^+ \mathrm{e}^{-\gamma t}, t\geq 0.
\end{multline}
where $C_{max} = \max_{i\in n} \sum_{j}^{m} C_{ij} $. 
\end{theorem}

\begin{proof}
Let $\mathcal{G} = C_{max} w_{max}+ g_{max}$, where $\|\bm{g}(\bm{x}(t),\bm{x}(t-r)) \|\leq g_{max}$,
and $\iota \leq  \frac{\mathcal{G}}{\eta} + 
      \beta ( \|\bm{\phi} \|_{\infty} -\frac{\mathcal{G}}{\delta})^+ $.
The proof can be easily obtained analogously to that of Theorem \ref{thm:expenential}. 
\end{proof}

The construction of the positive constants expect to $g_{max}$ can be done in the same way of Theorem \ref{thm:expenential}. 
To find $g_{max}$, we set the first function $H_1(g_{max})$: 
\begin{equation}
\label{eq:1}
    \| \bm{\xi}_{\bm{\phi}} \|_{\infty} \leq H_1(g_{max}).
\end{equation}
where $H_1(g_{max}) = \frac{\mathcal{G}}{\eta} + 
      \beta ( \|\bm{\phi} \|_{\infty} -\frac{\mathcal{G}}{\delta})^+ $.
For $\bm{g}(\bm{x}(t),\bm{x}(t-r))$, applying \eqref{eq:1}: 
\begin{equation*}
    \|\bm{x}(t)\|_{\infty} , \, \|\bm{x}(t-r)\|_{\infty} \leq H_1(g_{max}),
\end{equation*}
We have the second function $H_2(g_{max})$:
\begin{equation*}
\label{eq:2}
    \| \bm{g}(\bm{x}(t),\bm{x}(t-r)) \|_{\infty} \leq H_2(g_{max}).
\end{equation*}
By solving the inequation: $H_2(g_{max}) \leq g_{max}$, we can obtain $g_{max}$.

%reduce to T
\begin{theorem}
\label{thm:reduceT_nonlinear}
Given an initial function $\bm{\phi}$ and the equilibrium $\bm{x_e}=\bm{0}$,
if we know $\beta$, $\gamma$, $\delta$ and $\eta$, let $\mathfrak{r}_1=\frac{\mathcal{G}}{\eta} $ and $\mathfrak{r}_2 = \beta ( \|\bm{\phi} \|_{\infty} -\frac{\mathcal{G}}{\delta})$, then for any given $\epsilon >0$,
there exists a time bound $T^*$ defined by 
\begin{equation}
    T^* = \max\{ 0, \inf \{ T \mid \forall t\geq T : \mathfrak{r}_2^+ \mathrm{e}^{-\gamma t}<\epsilon \}\}
\end{equation}
the solution of systems \ref{dde:linearDDE} satisfies: for any $T \geq T^*$, 
$\|\bm{\xi}_{\bm{\phi}}(T)-\bm{x_e}\|_{\infty}- \mathfrak{r}_1 < \epsilon$,
then the differential invariant of the system \ref{dde:linearDDE} is equivalent to 
$T$-differential invariant. 
\end{theorem}
\begin{proof}
The proof is similar to that of Theorem \ref{thm:reduceT}.
\end{proof}

% add basin to guarantee globally 



% extend to multiple delay term in eq
 

 




==> proof.tex <==
\appendix
\section{Proof of Theorem~\ref{thm:invariant_sound}}\label{apx:A}

\begin{proof}
\textbf{Termination}:  Obviously, the algorithm must terminate as the loop is executed at most  $\lceil \frac{T^*}{\tau} \rceil$ times. 

\textbf{Soundness}: (i) If the algorithm returns the result at line 6, we have $\mathrm{R}_{P_i(q)} \subseteq P_i(q)\cup \mathfrak{B}(\bm{0},\mathfrak{r}_1 +\epsilon) $, then 
        \begin{align*}
        P_{i+1}(q)\cup \mathfrak{B}(\bm{0},\mathfrak{r}_1 +\epsilon) & =  P_{i}(q)\cup \mathrm{R}_{P_i(q)}\cup \mathfrak{B}(\bm{0},\mathfrak{r}_1 +\epsilon) \\
             &\subseteq  P_i(q)\cup \mathfrak{B}(\bm{0},\mathfrak{r}_1 +\epsilon) .
        \end{align*}
    By recursion,  $P_i(q)\cup \mathfrak{B}(\bm{0},\mathfrak{r}_1 +\epsilon)$ is an over-approximation of the reachable set over the infinite time horizon from the initial set for system \eqref{dde:linearDDE}, i.e.,  $P_i(q)\cup (\mathfrak{B}(\bm{0},\mathfrak{r}_1 +\epsilon)\cap \mathcal{S}_q )$  is a safe differential invariant for system \eqref{dde:linearDDE}. 
      (ii) If the algorithm terminates at line 15,  evidently $P_i(q)$ is a safe over-approximate reachable set over time horizon $[0, T^*]$ from the initial set for system \eqref{dde:linearDDE}. By Theorem \ref{thm:reduceT} and Lemma \ref{lem:attractor}, $P_i(q)\cup (\mathfrak{B}(\bm{0},\mathfrak{r}_1 +\epsilon)\cap \mathcal{S}_q )$  is a safe differential invariant for  system \eqref{dde:linearDDE}. 
\end{proof}


\section{Proof of Theorem~\ref{thm:framework_sound}}\label{apx:B}

\begin{proof}
We first prove that $I^*$ is a global invariant of $\mathcal{H}^*$ if  Algorithm \ref{alg:switch_controller} terminates and returns $\mathcal{H}^*=(Q, X, U^*, I^*, \Xi^* , F , E,D, G^*, R )$, i.e., the conditions (c1) and (c2) in Definition \ref{def:inductive_invariant} hold.
From line \ref{line:In} in Algorithm \ref{alg:switch_controller}, Definition \ref{def:diff_invariant} and the soundness of Algorithm \ref{alg:Invariant}, we have $I^*(q)$ is a differential invariant of $(\Xi^*(q),f_q,I(q)$, then (c1) holds.
Let $e=(q,q')\in E$, and $\bm{\xi}_{\bm{\phi}}^\mathbf{w}(t)\in G^*(e)$. 
From line \ref{line:kn}, \ref{line:In} in Algorithm \ref{alg:switch_controller} we have
\begin{align*}
\{  \bm{\phi} \mid    \exists e=(q', q)\in E,  \
    \bm{\phi}=R(e, \mathbf{x}) \wedge  \mathbf{x}\in\widetilde{G}(e)
\} \subseteq I^*(q),
\end{align*}
and from line \ref{line:G} have that $G^*_n(e)\gets$ \textbf{BackReach}($\widetilde{G}_n(e)$,   $D(e)$,   $I_n(q)$, $\bm{\rho},\tau$),
then (c2) holds. Thus, we have proved $I^*$ is a global invariant of $\mathcal{H}^*$.

Then, we prove the (r1), (r2) and (r3) in Problem \ref{prob:synthesis}.
Since each $I_n(q)$ is calculated by Algorithm \ref{alg:Invariant}, which guaranteed the invariant $I_n(q)$ is safe, thus $\mathcal{H}^*$ is safe, i.e., (r1) holds.
In Algorithm \ref{alg:switch_controller}, line \ref{line:xi} makes $\Xi^* \subseteq \Xi \cap \mathcal{S}$, line \ref{line:I_refine} makes $I^* \subseteq I$.
From line \ref{line:u}, and $I^* \subseteq I$, then $U^* \subseteq U$.
For any $e\in E$, $\mathbf{x}(t)\in G^*(e)$, then $\mathbf{x}(t+D(e))\in \widetilde{G}(e)$,
from line \ref{line:g}, \ref{line:G} then $\mathbf{x}(t+D(e))\in G(e)\cap I^*(q)$. Therefore, (r2) holds.
Actually, $I^*$ contains all the safe and real trajectory of $\mathcal{H}$, thus if $\mathcal{H}$ is non-blocking in the safe set $\mathcal{S}$, then $\mathcal{H}^*$ is also non-blocking, i.e., (r3) holds. 

Above all, we have prove this theorem.
\end{proof}




